Partial Measurements of Quantum Systems

Projective measurement is a commonly used assumption in quantum mechanics. However, advances in quantum measurement techniques allow for partial measurements, which accurately estimate state information while keeping the wavefunction intact. In this dissertation, we employ partial measurements to study two phenomena. First, we investigate an uncertainty relation -- in the style of Heisenberg's 1929 thought experiment -- which includes partial measurements in addition to projective measurements. We find that a weak partial measurement can decrease the uncertainty between two incompatible (non-commuting) observables. In the second study, we investigate the foundation of irreversible dynamics resulting from partial measurements. We do so by comparing the forward and time-reversed probabilities of measurement outcomes resulting from post-selected feedback protocols with both causal and reversed-causal order. We find that the statistics of partial measurements produce entropy in accordance with generalized second laws of thermodynamics. We perform these experiments using superconducting qubits. This dissertation also describes the fabrication process for these devices and details a novel fabrication technique that allows fast, single-step lithography of Josephson-junction superconducting circuits. The technique simplifies processing by utilizing a direct-write photolithography system, in contrast to traditional electron-beam lithography. Despite their large lithographic area, Josephson junctions made with this method have low critical currents and high coherence times.

==> bibExtra.tex <==
%
\bibitem [{\citenamefont {{Yunger Halpern}}(2017)}]{NYH_17_Jarzynski}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {{Yunger Halpern}}},\ }\bibfield  {title} {\bibinfo {title} {{Jarzynski-like
  equality for the out-of-time-ordered correlator}},\ }\href
  {https://doi.org/10.1103/PhysRevA.95.012120} {\bibfield  {journal} {\bibinfo
  {journal} {Physical Review A}\ }\textbf {\bibinfo {volume} {95}},\ \bibinfo
  {pages} {1} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%

\bibitem [{\citenamefont {Yunger~Halpern}\ \emph {et~al.}(2018)\citenamefont
  {Yunger~Halpern}, \citenamefont {Swingle},\ and\ \citenamefont
  {Dressel}}]{NYH_18_Quasiprobability}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Yunger~Halpern}}, \bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Swingle}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Dressel}},\ }\bibfield  {title} {\bibinfo {title} {Quasiprobability behind
  the out-of-time-ordered correlator},\ }\href
  {https://doi.org/10.1103/PhysRevA.97.042105} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo
  {pages} {042105} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%


\bibitem [{\citenamefont {Swingle}\ and\ \citenamefont
  {Yunger~Halpern}(2018)}]{Swingle_18_Resilience}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B.}~\bibnamefont
  {Swingle}}\ and\ \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Yunger~Halpern}},\ }\bibfield  {title} {\bibinfo {title} {Resilience of
  scrambling measurements},\ }\href
  {https://doi.org/10.1103/PhysRevA.97.062113} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {97}},\ \bibinfo
  {pages} {062113} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%

\bibitem [{\citenamefont {Gonz\'alez~Alonso}\ \emph {et~al.}(2019)\citenamefont
  {Gonz\'alez~Alonso}, \citenamefont {Yunger~Halpern},\ and\ \citenamefont
  {Dressel}}]{GonzalezAlonso_19_Out}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont
  {Gonz\'alez~Alonso}}, \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Yunger~Halpern}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Dressel}},\ }\bibfield  {title} {\bibinfo {title}
  {Out-of-time-ordered-correlator quasiprobabilities robustly witness
  scrambling},\ }\href {https://doi.org/10.1103/PhysRevLett.122.040404}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. Lett.}\ }\textbf
  {\bibinfo {volume} {122}},\ \bibinfo {pages} {040404} (\bibinfo {year}
  {2019})}\BibitemShut {NoStop}%

\bibitem [{\citenamefont {Dressel}\ \emph {et~al.}(2018)\citenamefont
  {Dressel}, \citenamefont {Gonz\'alez~Alonso}, \citenamefont {Waegell},\ and\
  \citenamefont {Yunger~Halpern}}]{Dressel_18_Strengthening}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Dressel}}, \bibinfo {author} {\bibfnamefont {J.~R.}\ \bibnamefont
  {Gonz\'alez~Alonso}}, \bibinfo {author} {\bibfnamefont {M.}~\bibnamefont
  {Waegell}},\ and\ \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
  {Yunger~Halpern}},\ }\bibfield  {title} {\bibinfo {title} {Strengthening weak
  measurements of qubit out-of-time-order correlators},\ }\href
  {https://doi.org/10.1103/PhysRevA.98.012132} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo {volume} {98}},\ \bibinfo
  {pages} {012132} (\bibinfo {year} {2018})}\BibitemShut {NoStop}%

\bibitem [{\citenamefont {Mohseninia}\ \emph {et~al.}(2019)\citenamefont
  {Mohseninia}, \citenamefont {Alonso},\ and\ \citenamefont
  {Dressel}}]{Mohseninia_19_Optimizing}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R.}~\bibnamefont
  {Mohseninia}}, \bibinfo {author} {\bibfnamefont {J.~R.~G.}\ \bibnamefont
  {Alonso}},\ and\ \bibinfo {author} {\bibfnamefont {J.}~\bibnamefont
  {Dressel}},\ }\bibfield  {title} {\bibinfo {title} {Optimizing measurement
  strengths for qubit quasiprobabilities behind out-of-time-ordered
  correlators},\ }\href {https://doi.org/10.1103/PhysRevA.100.062336}
  {\bibfield  {journal} {\bibinfo  {journal} {Phys. Rev. A}\ }\textbf {\bibinfo
  {volume} {100}},\ \bibinfo {pages} {062336} (\bibinfo {year}
  {2019})}\BibitemShut {NoStop}%

\bibitem [{\citenamefont {Arvidsson-Shukur}\ \emph {et~al.}(2020)\citenamefont
  {Arvidsson-Shukur}, \citenamefont {Yunger~Halpern}, \citenamefont {Lepage},
  \citenamefont {Lasek}, \citenamefont {Barnes},\ and\ \citenamefont
  {Lloyd}}]{DRMAS_19_Quantum}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {D.~R.~M.}\
  \bibnamefont {Arvidsson-Shukur}}, \bibinfo {author} {\bibfnamefont
  {N.}~\bibnamefont {Yunger~Halpern}}, \bibinfo {author} {\bibfnamefont
  {H.~V.}\ \bibnamefont {Lepage}}, \bibinfo {author} {\bibfnamefont {A.~A.}\
  \bibnamefont {Lasek}}, \bibinfo {author} {\bibfnamefont {C.~H.~W.}\
  \bibnamefont {Barnes}},\ and\ \bibinfo {author} {\bibfnamefont
  {S.}~\bibnamefont {Lloyd}},\ }\bibfield  {title} {\bibinfo {title} {Quantum
  advantage in postselected metrology},\ }\href
  {https://doi.org/10.1038/s41467-020-17559-w} {\bibfield  {journal} {\bibinfo
  {journal} {Nature Communications}\ }\textbf {\bibinfo {volume} {11}},\
  \bibinfo {pages} {3775} (\bibinfo {year} {2020})}\BibitemShut {NoStop}%

  % Added by hand by JTM
\bibitem [{\citenamefont {Arvidsson-Shukur}(2020)}]{Arvidsson-Shukur2020}
\BibitemOpen
\bibfield  {author} 
{\bibinfo {author} {\bibfnamefont {D.~R.~M.}\ \bibnamefont
		{{Arvidsson-Shukur}}}
	, \bibinfo {author} {\bibfnamefont {J.~C.}\ \bibnamefont
		{{Drori}}}
	,\ and\ \bibinfo {author} {\bibfnamefont {N.}~\bibnamefont
		{{Yunger Halpern}}},\ }
\bibfield  {title} {\bibinfo {title} {{Conditions tighter than 
			noncommutation needed for nonclassicality}},\ }
\href@noop {} {\bibfield  {journal}
	\bibinfo  {journal} {arXiv e-prints}\ ,\ \bibinfo {eid} {arXiv:2009.04468}
	(\bibinfo {year} {2020})},\ \Eprint {https://arxiv.org/abs/2009.04468}
{arXiv:2009.04468 [quant-ph]} \BibitemShut {NoStop}%

==> bin/embedfonts <==
#!/usr/bin/env perl
use strict;

my $input = shift( @ARGV );
my $output = shift( @ARGV );

print "Fonts before\n";
print `pdffonts $input`;

system("gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=letter -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$output -f $input");

print "\n";
print "Fonts after\n";
print `pdffonts $output`;

exit(0);


==> bin/joinpdf <==
#!/usr/bin/env perl
use strict;
use warnings;

##
# check for args < 2, just assume
# if 1 (i.e., help,etc.) are included
##
sub checkhelp($);
sub checkexists($);
sub checkgs();

## check to see if ghostscript is installed
checkgs();

checkhelp( \@ARGV );

##
# get files
##
my $output = $ARGV[ 0 ];
my @filestemp = @ARGV[1..(@ARGV-1)];
my $files  = join( ' ', checkexists( \@filestemp ));

`gs -dBATCH -dNOPAUSE -q -sDEVICE=pdfwrite -sOutputFile=$output $files`;

exit( 0 );


##
# takes in all env args 
##
sub checkhelp( $ )
{
   my $arr = shift( @_ );
   if( @$arr < 2 )
   {
      print STDOUT "<outputfile> <joinfiles> [more join files]\n";
      exit( 0 );
   }
   return;
}

##
# check for existence of all files, skip otherwise
##
sub checkexists( $ )
{
   my $arr = shift;
   my @exist;
   for my $file ( @$arr )
   { 
      chomp( $file );
      if( -e $file )
      {
         print "joining $file\n";
         push( @exist, $file );
      }
      else
      {
         print "File \"$file\" doesn't exist, skipping\n";
      }
   }
   if( @exist < 1 )
   {
      print( "Not enough files actually exist, try again!\n" );
      exit( -1 );
   }
   return( @exist  );
}

sub checkgs()
{
   if( `which gs` eq '' )
   {
      print STDERR "\nERROR: requires ghostscript, install from http://ghostscript.com\n";
      exit( -1 );
   }
}


==> bin/knitr2tex <==
#!/usr/bin/env ruby

require 'optparse'

options = {}
OptionParser.new do |opt|
  opt.on('-o', '--output FILE') { |o| options[:output] = o }
  opt.on('--cachepath PATH') { |o| options[:cachepath] = o }
  opt.on('--figurepath PATH') { |o| options[:figurepath] = o }
end.parse!

tex_filename = options[:output]
knitr_filename = ARGV.pop

raise "no knitr file given" unless knitr_filename
raise "no such file: #{knitr_filename}" unless File.exist?(knitr_filename)

unless tex_filename then
  tex_filename = File.basename(knitr_filename, File.extname(knitr_filename)) + ".tex"
end

cachedir_opt = ""
if options[:cachepath] then
  cachedir_opt = " knitr::opts_chunk[['set']](cache.path='#{options[:cachepath]}');"
end

figuredir_opt = ""
if options[:figurepath] then
  figuredir_opt = " knitr::opts_chunk[['set']](fig.path='#{options[:figurepath]}');"
end

cmd = "Rscript -e \"library(knitr); knitr::opts_knit\\$set(concordance = TRUE);#{cachedir_opt}#{figuredir_opt} knitr::knit(input = '#{knitr_filename}', output = '#{tex_filename}', quiet = TRUE);\""

if system(cmd) then
  # success!
else
  # It failed, delete the file because it is not valid
  File.delete(tex_filename)
end

exit($?.exitstatus)

